Evaluating gesture generation in a large-scale open challenge: The GENEA Challenge 2022

This paper reports on the second GENEA Challenge to benchmark data-driven automatic co-speech gesture generation. Participating teams used the same speech and motion dataset to build gesture-generation systems. Motion generated by all these systems was rendered to video using a standardised visualisation pipeline and evaluated in several large, crowdsourced user studies. Unlike when comparing different research papers, differences in results are here only due to differences between methods, enabling direct comparison between systems. The dataset was based on 18 hours of full-body motion capture, including fingers, of different persons engaging in a dyadic conversation. Ten teams participated in the challenge across two tiers: full-body and upper-body gesticulation. For each tier, we evaluated both the human-likeness of the gesture motion and its appropriateness for the specific speech signal. Our evaluations decouple human-likeness from gesture appropriateness, which has been a difficult problem in the field. The evaluation results show some synthetic gesture conditions being rated as significantly more human-like than 3D human motion capture. To the best of our knowledge, this has not been demonstrated before. On the other hand, all synthetic motion is found to be vastly less appropriate for the speech than the original motion-capture recordings. We also find that conventional objective metrics do not correlate well with subjective human-likeness ratings in this large evaluation. The one exception is the Fr\'echet gesture distance (FGD), which achieves a Kendall's tau rank correlation of around $-0.5$. Based on the challenge results we formulate numerous recommendations for system building and evaluation.

==> conditions_table.tex <==
\begin{table*}
%\small
\centering
\caption{Conditions participating in the evaluation. Conditions are ordered based on their median human-likeness scores from higher to lower (see Table \ref{tab:stats}).
For teams (but not for baselines) we cite the respective system-description paper, if available.
The following abbreviations were used:
\textit{AR} for ``Auto-regression'',
\textit{CNN} for ``Convolutional Neural Network'',
\textit{RNN} for ``Recurrent Neural Network'',
\textit{SA} for ``Neural self-attention'' (e.g., Transformers), \textit{GANs} for ``Generative adversarial networks or adversarial loss terms'',
\textit{VAEs} for ``Variational auto-encoders'',
\textit{MM} for ``Motion matching'',
\textit{Frame-wise} for ``Generating output frame-by-frame'', \textit{Stoch.\ output} for ``Stochastic output'' (different output possible even if the inputs are the same),
and \textit{Smoothed} for ``Smoothing was applied''.}
\small%
\begin{tabular}{@{}lll|ccc|c|ccccl|ccc@{}}
\toprule 
 & \multicolumn{2}{c|}{Per-tier} & \multicolumn{3}{c|}{Inputs used} & Hands & \multicolumn{5}{c|}{Techniques used} & Frame- & Stoch. & Smoo- \tabularnewline
Baseline or team name & \multicolumn{2}{c|}{label} & Aud. & Text & Sp. ID & Fixed & AR & RNNs & SA & VAEs & Other & wise & output & thed\tabularnewline
%\midrule
%Natural motion & \cmark & \cmark & \cmark & \multicolumn{7}{c@{}}{Not relevant} \tabularnewline
\midrule 
GestureMaster [\citeauthor{anon2022gesturemaster}] & FSA & USQ & \cmark & \cmark & \cmark &  & &  &  &  & Hand-crafted rules, MM &  &  & \cmark\tabularnewline
Forgerons [\citeauthor{ghorbani2022exempler}] & FSC & USO & \cmark &  &  & \cmark & \cmark & \cmark &  & \cmark &  & \cmark & \cmark &   \tabularnewline
DeepMotion [\citeauthor{lu2022deepmotion}] & FSI & USJ & \cmark & \cmark &  & \cmark & \cmark &  & \cmark & \cmark & CNNs & \cmark & \cmark & \tabularnewline
DSI [\citeauthor{saleh2022hybrid}] & FSF &  & \cmark &  &  &  & \cmark & \cmark & \cmark &  &  &  &  & \tabularnewline
UEA Digital Humans [\citeauthor{windle2022uea}] & FSG & USM & \cmark & \cmark & \cmark &  & & \cmark &  &  &  & \cmark &  & \tabularnewline
ReprGesture [\citeauthor{yang2022reprgesture}] & & USN & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & CNNs, GANs &  &  & \cmark\tabularnewline
IVI Lab [\citeauthor{chang2022ivi}] & FSH & USK & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark &  &  &  & \cmark & \cmark & \cmark\tabularnewline
FineMotion [\citeauthor{korzun2022recell}] & FSD & & \cmark & \cmark &  &  & \cmark & \cmark &  &  &  & \cmark &  & \cmark\tabularnewline
Murple AI lab (no paper submitted) & \multicolumn{2}{c|}{Not revealed} & \cmark &  &  &  & \cmark & \cmark &  &  & Normalising flows & \cmark & \cmark & 
\tabularnewline
Text-only baseline
%[\citeauthor{yoon2019robots}]
& FBT & UBT & & \cmark & & \cmark & \cmark & \cmark  &  &  &  & \cmark &  & \cmark \tabularnewline
Audio-only baseline
%[\citeauthor{kucherenko2019analyzing}]
& & UBA & \cmark &  &  & &  &  \cmark &  &  &  & \cmark &  & \cmark \tabularnewline
%\midrule 
TransGesture [\citeauthor{kaneko2022transgesture}] & & USL & \cmark &  & & \cmark  & \cmark & \cmark &  &  &  & \cmark &  & \cmark\tabularnewline
\bottomrule
\end{tabular}
\label{tab:conditions}
\end{table*}

==> old/conditions_table.tex <==
\begin{table}
\small
\centering
\caption{Conditions participating in the evaluation. Teams are sorted alphabetically by name. The anonymised IDs of submitted entries begin with the letter `S' followed by a second, randomly-assigned letter in the range A through E, but which letter is associated which each team is not revealed in order to preserve anonymity. $\dagger$ indicates a use of word vectors pretrained on external data.}
\begin{tabular}{@{}lll|cc|cc|c@{}}
\toprule 
 &  &  & \multicolumn{2}{c|}{Inputs used} & \multicolumn{2}{c|}{Representation or features} & Stochastic \\
% &  &  & \multicolumn{2}{c|}{Inputs used?} & \multicolumn{3}{c|}{External data used?} & \multicolumn{2}{c|}{Representation or features} & Stochastic \\
\cmidrule{4-7}
%Name or description & Origin & ID & Aud. & Text & Aud. & Text & Motion & Input & Output & output? \\
Name or description & Origin & ID & Aud. & Text & Input speech & Motion & output? \\
\midrule
Natural motion & - & N & \cmark & \cmark & -- & -- & \cmark\\
Mismatched motion & - & M & \xmark & \xmark & -- & -- & \cmark\\
\midrule
Audio-only baseline & \citeauthor{kucherenko2019analyzing} \cite{kucherenko2019analyzing} & BA & \cmark & \xmark & MFCC & Exp.\ map & \xmark\\
Text-only baseline & \citeauthor{yoon2019robots} \cite{yoon2019robots} & BT & \xmark & \cmark & FastText${}^\dagger$ & Rot.\ matrix & \xmark\\
\midrule
AlltheSmooth \cite{jinhong_lu_2020_4088376} & CSTR lab, UEDIN, Scotland & S... & \cmark & \xmark & MFCCs & Joint pos.& \xmark\\
Edinburgh CVGU \cite{kunkun_pang_2020_4090879} & CVGU lab, UEDIN, Scotland & S... & \cmark & \cmark & BERT${}^\dagger$ \& mel-spectr. & Rot.\ matrix & \cmark\\
FineMotion \cite{vladislav_korzun_2020_4088609} & ABBYY lab, MIPT, Russia & S...& \cmark & \cmark & GloVe${}^\dagger$ \& mel-spectr. & Exp.\ map & \xmark\\
Nectec \cite{ausdang_thangthai_2020_4088629} & \begin{tabular}{@{}l@{}}HCCR unit, NECTEC, \\Thailand\end{tabular} & S...& \cmark & \cmark & \begin{tabular}{@{}c@{}}Phoneme, Spacy word \\vecs.${}^\dagger$, MFCCs, \& prosody\end{tabular} & \begin{tabular}{@{}c@{}}Exp.\ map\end{tabular} & \xmark\\
StyleGestures \cite{simon_alexanderson_2020_4088600} & TMH division, KTH, Sweden & S... & \cmark & \xmark & mel-spectr. & Exp.\ map & \cmark\\
\bottomrule
\end{tabular}
\label{tab:conditions}
\end{table}

==> old/old_table_version/table1.tex <==
\begin{table*}
%\small
\centering
\caption{Conditions participating in the evaluation. Teams are ordered alphabetically. The following non-standard abbreviations were used: \textit{AR} for ``Auto-regression'',
%\textit{CNN} for ``Convolutional Neural Network'', \textit{RNN} for ``Recurrent Neural Network'',
\textit{SA} for ``Neural self-attention'' (e.g., Transformers), \textit{GANs} for ``Generative adversarial networks or adversarial loss terms'',
%\textit{VAEs} for ``Variational auto-encoders'',
%\textit{H.\ rules} for ``Hand-crafted rules'',
and \textit{MM} for ``Motion matching'',
%The following column names were shortened:
\textit{Frame-wise} for ``Generating output frame-by-frame'', \textit{Stoch.\ output} for ``Stochastic output'',
%(different output possible even if the inputs are the same),
and \textit{Smoothed} for ``Smoothing was applied''.}
\small%
\begin{tabular}{@{}ll|ccc|ccccl|ccc@{}}
\toprule 
Baseline or team name & Label & \multicolumn{3}{c|}{Inputs used} & \multicolumn{5}{c|}{Techniques used} & Frame- & Stoch. & Smoo\tabularnewline
 & & Aud. & Text & Sp.\ ID & AR & RNNs & SA & VAEs & Other & wise & output & thed\tabularnewline
%\midrule
%Natural motion & \cmark & \cmark & \cmark & \multicolumn{7}{c@{}}{Not relevant} \tabularnewline
\midrule 
Audio-only baseline \cite{kucherenko2019analyzing} & UBA & \cmark &  &  &  &  \cmark &  &  &  & \cmark &  & \cmark \tabularnewline
Text-only baseline \cite{yoon2019robots} & UBT/FBT & & \cmark &  & \cmark & \cmark  &  &  &  & \cmark &  & \cmark \tabularnewline
\midrule 
DeepMotion \cite{lu2022deepmotion} & USJ/FSI & \cmark & \cmark &  & \cmark &  & \cmark & \cmark & CNNs & \cmark & \cmark & \tabularnewline
DSI \cite{saleh2022hybrid} & FSF & \cmark &  &  & \cmark & \cmark & \cmark &  &  &  &  & \tabularnewline
FineMotion \cite{korzun2022recell} & FSD & \cmark & \cmark &  & \cmark & \cmark &  &  &  & \cmark &  & \cmark\tabularnewline
Forgerons \cite{ghorbani2022exempler} & USO/FSC & \cmark &  &  & \cmark & \cmark &  & \cmark &  & \cmark & \cmark &   \tabularnewline
GestureMaster \cite{zhou2022gesturenaster} & USQ/FSA & \cmark & \cmark & \cmark &  &  &  &  & Hand-crafted rules, MM &  &  & \cmark\tabularnewline
IVI Lab \cite{chang2022ivi} & USK/FSH & \cmark & \cmark & \cmark & \cmark & \cmark &  &  &  & \cmark & \cmark & \cmark\tabularnewline
Murple AI lab & USP/FSB & \cmark &  &  & \cmark & \cmark &  &  & Normalizing Flows & \cmark & \cmark & 
\tabularnewline
ReprGesture \cite{yang2022reprgesture} & USN & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & CNNs, GANs &  &  & \cmark\tabularnewline
TransGesture \cite{kaneko2022transgesture} & USL & \cmark &  &  & \cmark & \cmark &  &  &  & \cmark &  & \cmark\tabularnewline
UEA Digital Humans \cite{windle2022uea} & USM/FSG & \cmark & \cmark & \cmark &  & \cmark &  &  &  & \cmark &  & \tabularnewline
\bottomrule
\end{tabular}
\label{tab:conditions}
\end{table*}

==> old/results_table.tex <==
\begin{table}
\begin{minipage}{.53\columnwidth}
    \centering
    \caption{Summary statistics of user-study ratings for all conditions in the two studies, with 0.01-level confidence intervals. The human-likeness of M was not evaluated explicitly, since it uses the same motion clips as N.}
    \label{tab:results}
    %\resizebox{\columnwidth}{!}{%
        \begin{tabular}{@{}l|cc|cc@{}}
        \toprule
        & \multicolumn{2}{c|}{Human-likeness} & \multicolumn{2}{c}{Appropriateness}\\
        ID & Median & Mean & Median & Mean\\
        \midrule
        N & $72\in{}[70,\,75]$ & $67.6\pm{}1.8$ & $81\in{}[79,\,83]$ & $73.8\pm{}1.8$\\
        M & \tqdb{} & \tqdb{} & $56\in{}[53,\,59]$ & $53.3\pm{}2.0$\\
        BA & $46\in{}[44,\,49]$ & $46.2\pm{}1.7$ & $40\in{}[38,\,41]$ & $40.4\pm{}1.8$\\
        BT & $55\in{}[53,\,58]$ & $54.6\pm{}1.8$ & $38\in{}[35,\,40]$ & $38.5\pm{}1.9$\\
        SA & $38\in{}[35,\,41]$ & $40.1\pm{}1.9$ & $35\in{}[31,\,37]$ & $36.4\pm{}1.9$\\
        SB & $52\in{}[50,\,55]$ & $52.8\pm{}1.9$ & $43\in{}[40,\,45]$ & $43.3\pm{}2.0$\\
        SC & $57\in{}[55,\,60]$ & $55.8\pm{}1.9$ & $50\in{}[48,\,52]$ & $50.6\pm{}1.9$\\
        SD & $60\in{}[57,\,61]$ & $58.8\pm{}1.7$ & $49\in{}[46,\,50]$ & $48.1\pm{}1.9$\\
        SE & $49\in{}[47,\,51]$ & $49.6\pm{}1.8$ & $47\in{}[44,\,49]$ & $45.9\pm{}1.8$\\
        \bottomrule
        \end{tabular}
    %}
\end{minipage}
\hfill%
%\hspace{1mm}
\begin{minipage}{.45\columnwidth}
    %\vspace*{1.06cm}
    \caption{Results from the objective evaluations. The Hellinger distance between natural and synthetic speed profiles was computed for the two wrist joints, since hand motion is of central importance for co-speech gestures.}
    \label{tab:obj_evaluations}
    \centering
    %\resizebox{\columnwidth}{!}{%
        \begin{tabular}{@{}l|lcc@{}}
        \toprule
         &  & \multicolumn{2}{c@{}}{Hellinger distance} \\
        ID & Jerk & Left & Right \\
        \midrule
        N & 151.52 $\pm$ 35.57 & 0\hphantom{.000} & 0\hphantom{.000} \\
         &  &  &  \\
        BA & \hphantom{0}65.59 $\pm$ \hphantom{0}4.42 & 0.084 & 0.090\\
        BT & \hphantom{0}45.84 $\pm$ \hphantom{0}2.14 & 0.130 & 0.096 \\
        SA & 132.37 $\pm$ 27.64 & 0.064 & 0.059 \\
        SB & 189.39 $\pm$ \hphantom{0}4.66 & 0.126 & 0.114\\
        SC & \hphantom{0}84.44 $\pm$ \hphantom{0}8.48 & 0.083 & 0.088 \\
        SD & \hphantom{0}72.06 $\pm$ \hphantom{0}7.91 & 0.073 & 0.062 \\
        SE & \hphantom{0}97.85 $\pm$ \hphantom{0}9.34 & 0.049 & 0.049 \\
        \bottomrule
        \end{tabular}
    %}
\end{minipage} 
\end{table}



==> old/template/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> old/template/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

